Energy Balancing of Covariate Distributions

Bias in causal comparisons has a direct correspondence with distributional imbalance of covariates between treatment groups. Weighting strategies such as inverse propensity score weighting attempt to mitigate bias by either modeling the treatment assignment mechanism or balancing specified covariate moments. This paper introduces a new weighting method, called energy balancing, which instead aims to balance weighted covariate distributions. By directly targeting distributional imbalance, the proposed weighting strategy can be flexibly utilized in a wide variety of causal analyses, including the estimation of average treatment effects and individualized treatment rules. Our energy balancing weights (EBW) approach has several advantages over existing weighting techniques. First, it offers a model-free and robust approach for obtaining covariate balance that does not require tuning parameters, obviating the need for modeling decisions of secondary nature to the scientific question at hand. Second, since this approach is based on a genuine measure of distributional balance, it provides a means for assessing the balance induced by a given set of weights for a given dataset. Finally, the proposed method is computationally efficient and has desirable theoretical guarantees under mild conditions. We demonstrate the effectiveness of this EBW approach in a suite of simulation experiments, and in studies on the safety of right heart catheterization and the effect of indwelling arterial catheters.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> section_02_methods/section_bootstrapping_old.tex <==


\subsection{Bootstrapping with energy balancing weights}
Standard nonparametric (balanced?) bootstrap:
\begin{itemize}
    \item For $b = 1, \cdots, B$:
    \begin{enumerate}
    \item Draw a new bootstrap sample with replacement $\{(Y_i^{*b}, A_i^{*b}, \bX_i^{*b})\}_{i=1}^n$, with balance constraints $\sum_{i=1}^n A_i^{*b}=n_1$ and $\sum_{i=1}^n (1-A_i^{*b})=n_0$.
    \item Estimate weights $(w_i^{*b})_{i=1}^n$ via propensity score modeling.
    \item Compute the bootstrapped WATE estimator:
    \[\widehat{\tau}_\bw^{*b} = \frac{1}{n_1}\sum_{i=1}^nw_i^{*b} Y_i^{*b} A_i^{*b} - \frac{1}{n_0}\sum_{i =1}^n w_i^{*b} Y_i^{*b} (1-A_i^{*b}).\]
    \end{enumerate}
    \item Use $(\widehat{\tau}_\bw^{*b})_{b=1}^B$ to estimate sampling distribution of the WATE estimator $\widehat{\tau}_\bw$.
\end{itemize}
\crd{Estimating the conditional sampling distribution $[\widehat{\tau}_\bw|\sum_{i=1}^n A_i = n_1]$?}

EBW bootstrap:
\begin{itemize}
    \item Compute energy-balancing weights $\bw_n^e$
    \item For $b = 1, \cdots, B$:
    \begin{enumerate}
    \item Draw a new bootstrap sample with replacement $\{(Y_i^{*b}, A_i^{*b}, \bX_i^{*b})\}_{i=1}^n$, weighted by EBW $\bw_n^e$ with balance constraints $\sum_{i=1}^n A_i^{*b}=n_1$ and $\sum_{i=1}^n (1-A_i^{*b})=n_0$.
    \item Compute the bootstrapped ATE estimator:
    \[\widehat{\tau}_{\bw_n^e}^{*b} = \frac{1}{n_1}\sum_{i=1}^n Y_i^{*b} A_i^{*b} - \frac{1}{n_0}\sum_{i =1}^n Y_i^{*b} (1-A_i^{*b}).\]
    \end{enumerate}
    \item Use $(\widehat{\tau}_{\bw_n^e}^{*b})_{b=1}^B$ to estimate sampling distribution of the EBW estimator $\widehat{\tau}_{\bw_n^e}$.
\end{itemize}
\crd{Thoughts:
\begin{itemize}
    \item Estimating the conditional sampling distribution $[\widehat{\tau}_\bw|\sum_{i=1}^n A_i = n_1, \bw_n^e]$?
    \item Computationally more efficient if $\bw_n^e$ is precomputed before bootstrapping... but would it underestimate uncertainty of estimator?
    \item How to gauge "best"? How well we estimate the sampling distribution of interest?
    \item Potential ways to make bootstrapping more efficient: importance sampling for bootstrapping CIs (Johns, 1998), importance resampling (Do \& Hall, 1991), balanced importance resampling (Booth, Hall \& Wood, 1993). But these don't seem to be dealing with an explicit change of measure. There must be something in the importance sampling literature, where one samples from a different proposal, but wishes to infer the sampling distribution rather than just the mean...
\end{itemize}
}

==> section_04_simulation/supplement_additional_simulation_results.tex <==



